Accelerating Deep Learning with Fixed Time Budget

The success of modern deep learning is attributed to two key elements: huge amounts of training data and large model sizes. Where a vast amount of data allows the model to learn more features, the large model architecture boosts the learning capability of the model. However, both these factors result in prolonged training time. In some practical applications such as edge-based learning and federated learning, limited-time budgets necessitate more efficient training methods. This paper proposes an effective technique for training arbitrary deep learning models within fixed time constraints utilizing sample importance and dynamic ranking. The proposed method is extensively evaluated in both classification and regression tasks in computer vision. The results consistently show clear gains achieved by the proposed method in improving the learning performance of various state-of-the-art deep learning models in both regression and classification tasks.

==> biographies/hamid.tex <==

% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{hamid.jpg}}]{Hamid Menouar} (SM’16) is a Senior Research and Development Expert at Qatar Mobility Innovations Center (QMIC), Qatar, where he leads the development of innovations in the area of smart cities and smart living.  
% Before moving to Qatar in 2010, Hamid worked for 8 years at Hitachi research lab in Sophia Antipolice, France, where he contributed and led research and development activities related to connected vehicles. During his experience with Hitachi, he has heavily contributed to the development of connected vehicles communication standards in Europe through an active participation at ETSI TC ITS and Car to Car Communication Consortium.  
% Hamid received the Engineering degree (M.S.) in computer science from the University of Science and Technology Houari Boumediene, Algiers, Algeria, in 2003, the DEA (M.S.) degree in systems and information technologies from the University of Technology of Compiegne, France, 2004, and the Ph.D. degree in computer science from Telecom ParisTech, Paris, France, in 2008. 
% \end{IEEEbiography}

\begin{wrapfigure}{l}{23mm} \includegraphics[width=1in,height=2.2in,clip,keepaspectratio]{biographies/hamid.jpg} \end{wrapfigure}
\textbf{Hamid Menouar} (SM’16) is a Senior Research and Development Expert at Qatar Mobility Innovations Center (QMIC), Qatar, where he leads the development of innovations in the area of smart cities and smart living. Before moving to Qatar in 2010, Hamid worked for 8 years at Hitachi research lab in Sophia Antipolice, France, where he contributed and led research and development activities related to connected vehicles. During his experience with Hitachi, he has heavily contributed to the development of connected vehicles communication standards in Europe through an active participation at ETSI TC ITS and Car to Car Communication Consortium. Hamid received the Engineering degree (M.S.) in computer science from the University of Science and Technology Houari Boumediene, Algiers, Algeria, in 2003, the DEA (M.S.) degree in systems and information technologies from the University of Technology of Compiegne, France, 2004, and the Ph.D. degree in computer science from Telecom ParisTech, Paris, France, in 2008. 


==> biographies/hamila.tex <==
% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{hamila.jpg}}]{Prof. Ridha Hamila} received the MSc, LicTech with distinction, and PhD degrees from Tampere University of Technology (TUT), Tampere, Finland, in 1996, 1999, and 2002, respectively. Dr. Hamila currently a Full Professor at the Department of Electrical Engineering, Qatar University, Qatar. From 1994 to 2002 he held various research and teaching positions at TUT within the Department of Information Technology, Finland. From 2002 to 2003 he was a System Specialist at Nokia research Center and Nokia Networks, Helsinki. From 2004 to 2009 he was with Emirates Telecommunications Corporation, UAE. Also, from 2004 to 2013 he was adjunct Professor at the Department of Communications Engineering, TUT. His current research interests include mobile and broadband wireless communication systems, Mobile Edge Computing, Internet of Everything, and Machine Learning. In these areas, he has published over 200 journal and conference papers most of them in the peered reviewed IEEE publications, filed seven US patents, and wrote numerous confidential industrial research reports.  Dr. Hamila has been involved in several past and current industrial projects, Ooreedo, Qatar National Research Fund, Finnish Academy projects, EU research and education programs. He supervised a large number of under/graduate students and postdoctoral fellows. He organized many international workshops and conferences. He is a Senior Member of IEEE.
% \end{IEEEbiography}


\begin{wrapfigure}{l}{23mm} \includegraphics[width=1in,height=2.4in,clip,keepaspectratio]{biographies/hamila.jpg} \end{wrapfigure}
\textbf{Ridha Hamila} received the MSc, LicTech with distinction, and PhD degrees from Tampere University of Technology (TUT), Tampere, Finland, in 1996, 1999, and 2002, respectively. Dr. Hamila is currently a Full Professor at the Department of Electrical Engineering, Qatar University, Qatar. From 1994 to 2002 he held various research and teaching positions at TUT within the Department of Information Technology, Finland. From 2002 to 2003 he was a System Specialist at Nokia research Center and Nokia Networks, Helsinki. From 2004 to 2009 he was with Emirates Telecommunications Corporation, UAE. Also, from 2004 to 2013 he was adjunct Professor at the Department of Communications Engineering, TUT. His current research interests include mobile and broadband wireless communication systems, Mobile Edge Computing, Internet of Everything, and Machine Learning. In these areas, he has published over 200 journal and conference papers most of them in the peered reviewed IEEE publications, filed seven US patents, and wrote numerous confidential industrial research reports.  Dr. Hamila has been involved in several past and current industrial projects, Ooreedo, Qatar National Research Fund, Finnish Academy projects, EU research and education programs. He supervised a large number of under/graduate students and postdoctoral fellows. He organized many international workshops and conferences. He is a Senior Member of IEEE.

==> biographies/khan.tex <==
% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{biographies/khan.jpg}}]{Muhammad Asif Khan} (SM'20) received the B.Sc. degree in Telecommunication Engineering from University of Engineering and Technology Peshawar, Pakistan (2009) and M.Sc. in Telecommunication Engineering from University of Engineering and Technology Taxila, Pakistan (2013). He received the Ph.D. degree in Electrical Engineering from Qatar University in 2020. He was a Researcher Assistant at Qatar University (2014-2015) and at Qatar Mobility Innovation Center (2016-2017). He is currently working as a postdoctoral researcher at Qatar University. His current research interests include wireless communication, mobile edge computing, and distributed machine learning. He is a Senior Member of IEEE and a Member of IET. For more detailed information, please visit his homepage: \url{http://www.asifk.me}.
% \end{IEEEbiography}


%% Other journals using picinpar package
% \parpic{\includegraphics[width=1in,clip,keepaspectratio]{biographies/khan.jpg}}
% \noindent {\bf Muhammad Asif Khan} received the B.Sc. degree in Telecommunication Engineering from University of Engineering and Technology Peshawar, Pakistan (2009) and M.Sc. in Telecommunication Engineering from University of Engineering and Technology Taxila, Pakistan (2013). He received the Ph.D. degree in Electrical Engineering from Qatar University in 2020. He was a Researcher Assistant at Qatar University (2014-2015) and at Qatar Mobility Innovation Center (2016-2017). He is currently working as a postdoctoral researcher at Qatar University. His current research interests include wireless communication, mobile edge computing, and distributed machine learning. He is a Senior Member of IEEE and a Member of IET.
% % For more detailed information, please visit his homepage: \url{http://www.asifk.me}.

% \authorbiography[scale=0.3,overhang=0pt,wraplines=9,imagewidth=3cm,imagepos=]{biographies/khan.jpg}{Muhammad Asif Khan}
% {received the B.Sc. degree in Telecommunication Engineering from University of Engineering and Technology Peshawar, Pakistan (2009) and M.Sc. in Telecommunication Engineering from University of Engineering and Technology Taxila, Pakistan (2013). He received the Ph.D. degree in Electrical Engineering from Qatar University in 2020. He was a Researcher Assistant at Qatar University (2014-2015) and at Qatar Mobility Innovation Center (2016-2017). He is currently working as a postdoctoral researcher at Qatar University. His current research interests include wireless communication, mobile edge computing, and distributed machine learning. He is a Senior Member of IEEE and a Member of IET. For more detailed information, please visit his homepage: \url{http://www.asifk.me}}

\begin{wrapfigure}{l}{23mm} \includegraphics[width=1in,height=2.4in,clip,keepaspectratio]{biographies/khan.jpg} \end{wrapfigure}
\small
\textbf{Muhammad Asif Khan} (SMIEEE) is a Research Scientist at Qatar Mobility Innovations Center (QMIC). He received a Ph.D. degree in Electrical Engineering from Qatar University (2020), an M.Sc. degree in Telecommunication Engineering from the University of Engineering and Technology Taxila, Pakistan (2013), and a B.Sc. degree in Telecommunication Engineering from the University of Engineering and Technology Peshawar, Pakistan (2009). He also serves/served as an associate editor (AE) of the IEEE Technology Policy and Ethics newsletter and guest editor at Frontiers in Communications and Networks. He also serves on the review panel of high-impact IEEE transactions and journals. He has also served/serving as a TPC member of major IEEE conferences including IEEE ICC, IEEE CCNC, IEEE SusTech, IEEE BigData, IEEE Sensors, IEEE ICASSP, etc. He has published more than 40 peer-reviewed articles in high-impact journals and international conferences. He is a Senior Member of the IEEE and a Member of IET. He is a chartered engineer (CEng) with the Engineering Council (EC-UK). His current research focuses on edge intelligence, distributed ML, computer vision, and cybersecurity. For more detailed information, please visit his homepage: \url{https://muasifk.github.io/}


==> figures/tab_settings.tex <==



\begin{table*}[ht]
\centering
\caption{Summary of experimental settings.}
% \resizebox{.98\columnwidth}{!}{
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1}
% \begin{tabular}{|p{1.5cm}|p{3cm}|p{3cm}|} \hline
% & \textbf{Classification} & \textbf{Regression} \\ [0.5em] \hline
% && \\[-0.5em]       
% Tasks  & Image classification  & Density estimation \\[0.5em]
% Datasets & CIFAR10  & ShanghaiTech Part B, CARPK \\[0.5em]
% Baselines & VGG16, ResNet18, MobileNet\_V2, Custom Nets (small, medium, large)  &MCNN, CMTL, CSRNet, TEDnet, ASNet, SASNet, and LCDnet. \\ [0.5em]
% Metrics & Accuracy & MAE, MSE \\ [0.5em] \hline
% \end{tabular}


%%%%%%%%%%%%%%%  Using bookstab
\begin{tabular}{|p{3cm}|p{5.5cm}p{5.5cm}|} \toprule
& \textbf{Classification} & \textbf{Regression} \\ \midrule
&& \\[-0.5em]       
Tasks  & Image classification  & Density estimation \\[0.5em]
Datasets & CIFAR10, CIFAR100  & ShanghaiTech-PB, CARPK \\[1em]
Baselines & VGG16, ResNet18, MobileNet\_V2, Custom Nets (small, medium, large)  &MCNN, CMTL, CSRNet, TEDnet, ASNet, SASNet, and DroneNet. \\ [2em]
Metrics & Accuracy & MAE, MSE \\ [0.5em]
Sampling ratio ($\alpha$) & \{0.3, 0.4\} & \{0.2, 0.3\}\\ [1.5em]
Optimizer & Adam & Adam \\ [0.2em] \bottomrule

\end{tabular}
% }
\label{tab_settings}
\end{table*}

==> tables/tab_results_accuracy.tex <==




\begin{table*}[!h]
\centering
\caption{Density Class detection using LCDnet.}
\label{tab:results_accuracy}
\begin{tabular}{p{2cm} p{2cm} p{2cm}  p{1cm} p{2cm} p{2cm} p{2cm} } \toprule
Crowd Density  &\multicolumn{2}{c}{DroneRGBT}  & &\multicolumn{2}{c}{CARPK}  \\ \cmidrule{2-3} \cmidrule{5-6}
        &Count range   &Accuracy (\%)  & &Count range &Accuracy \\ \midrule
Very Low     &0-20     &58.4            &  &0-20     &71.3 \\
Low          &21-50    &78.2            &  &21-50    &82.1 \\
Medium       &51-100   &83.9            &  &51-100   &79.5 \\
High         &101-403  &62.4            &  &101-200  &98.6 \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/tab_results_complexity.tex <==




\begin{table*}[!h]
\centering
\renewcommand*{\arraystretch}{1.5}
\caption{Comparison of \rev{proposed scheme (LCDnet trained with curriculum learning) against SOTA models} for number of parameters (in Million), GMACs, size (in MB), and inference time (in mili seconds) for fixed input size.}
\label{tab:results_complexity}
\begin{tabular}{p{2.5cm} ccccccc} \toprule
Model    &Output &Parameters (M)  &Size (MB)   &GMACs &\multicolumn{3}{c}{Inference Time (s)}  \\ \midrule 

& & & & &Server &Jetson Xavier &Jetson Nano \\ \midrule
CrowdCNN \cite{CrowdCNN_CVPR2015}    &1/4 &1.66 &6.65  &3.96 &0.071 &0.073 &0.23\\ % For 72x72 patch, Para=1.66, Size=6.65, GMACs=62.94
MCNN \cite{MCNN_CVPR2016}    & 1/4 &0.13 &0.53 &8.82   &0.05 &0.10 &0.21\\
CMTL  \cite{CMTL_AVSS2017}   &1/4 &2.45  &9.82 &39.82 &0.098 &0.31 &0.62\\ 
CSRNet \cite{CSRNet_CVPR2018}  &1/8   &16.26 &65.05  &135.4 &0.19 &1.01 &1.88\\
SANet \cite{SANet_ECCV2018}   &1/4 &0.25 &1.02  &8.97 &0.075 &0.12 &0.23\\
\textbf{LCDnet (ours)}   &\textbf{1/2} &\textbf{0.05}  &\textbf{0.21} &\textbf{4.85} &\textbf{0.006} &\textbf{0.05} &\textbf{0.10}\\ \bottomrule
\end{tabular}
\end{table*}

==> tables/tab_results_error.tex <==





\begin{table*}[!h]
\centering
\caption{Accuracy comparison of the \rev{proposed scheme (LCDnet trained with curriculum learning) against SOTA models} over DroneRGBT dataset \cite{DroneRGBT_dataset} and CARPK dataset \cite{CARPK_dataset}.}
\label{tab:results_error}
\begin{tabular}{cccccccccc} \toprule

Method  &\multicolumn{4}{c}{DroneRGBT}  & &\multicolumn{4}{c}{CARPK} \\ \cmidrule{2-5}  \cmidrule{7-10}
&MAE &GAME &SSIM &PSNR & &MAE &GAME &SSIM &PSNR\\ \midrule \midrule

\rev{CrowdCNN \cite{CrowdCNN_CVPR2015}} &\rev{26.6} &\rev{48.2} &\rev{0.52} &\rev{17.3} & &\rev{15.6} &\rev{49.1} &\rev{0.63}  &\rev{18.8} \\[0.2em]


MCNN \cite{MCNN_CVPR2016}            &17.9  &44.49 &0.54 &18.2 &   &10.3 &42.40 &0.76 &19.21 \\[0.2em]

\rev{
CMTL \cite{CMTL_AVSS2017}}            &\rev{18.1} &\rev{40.5} &\rev{0.53} &\rev{17.1} &   &\rev{10.2} &\rev{41.3} &\rev{0.73} &\rev{19.0} \\[0.2em]

CSRNet \cite{CSRNet_CVPR2018}        &7.6 &25.7 &0.72 &21.70 &   &6.12 &21.8 &0.82 &20.52\\[0.2em]

\khan{SANet \cite{SANet_ECCV2018}} &\rev{16.2} &\rev{34.5} &\rev{0.59} &\rev{19.4} & &\rev{9.8} &\rev{27.2} &\rev{0.76}  &\rev{19.8} \\[0.2em]

\textbf{LCDnet (ours)}       &\textbf{21.4} &\textbf{46.9} &\textbf{0.60} &\textbf{21.39} &   &\textbf{13.1} &\textbf{45.2} &\textbf{0.79} &\textbf{20.14} \\[0.2em]

\bottomrule
\end{tabular}
\end{table*}
